Adversarial Sample Detection for Deep Neural Network through Model Mutation Testing

Deep neural networks (DNN) have been shown to be useful in a wide range of applications. However, they are also known to be vulnerable to adversarial samples. By transforming a normal sample with some carefully crafted human imperceptible perturbations, even highly accurate DNN make wrong decisions. Multiple defense mechanisms have been proposed which aim to hinder the generation of such adversarial samples. However, a recent work show that most of them are ineffective. In this work, we propose an alternative approach to detect adversarial samples at runtime. Our main observation is that adversarial samples are much more sensitive than normal samples if we impose random mutations on the DNN. We thus first propose a measure of `sensitivity' and show empirically that normal samples and adversarial samples have distinguishable sensitivity. We then integrate statistical hypothesis testing and model mutation testing to check whether an input sample is likely to be normal or adversarial at runtime by measuring its sensitivity. We evaluated our approach on the MNIST and CIFAR10 datasets. The results show that our approach detects adversarial samples generated by state-of-the-art attacking methods efficiently and accurately.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> background.tex <==
\section{Background}\label{sec:back}
In this section, we first review the necessary background of this work (i.e., includes Deep Neural Networks (DNN) for classification and adversarial samples for DNN) and then define our problem.

\subsection{Deep Neural Networks} Deep learning systems are emerging in many different applications including computer vision, natural language processing, and malware detection. Different DNN architectures like Convolutional Neural networks (CNN) and Recurrent Neural Networks (RNN) have been proposed for different application scenarios. In this work, we focus on DNN classifiers which takes a given sample and labels the sample according (e.g., as certain object). In the following, we use $\mathbf{x}$ to denote an input sample for a DNN $f$. We use $c_\mathbf{x}$ to denote the ground-truth label of $\mathbf{x}$. Given an input sample $\mathbf{x}$ and a DNN $f$, we can obtain the label of the input $\mathbf{x}$ under $f$ by performing forward propagation. $\mathbf{x}$ is regarded as an \textit{adversarial sample} with respect to the DNN $f$ if $f(\mathbf{x})\neq c_\mathbf{x}$. $\mathbf{x}$ is regarded as a \textit{normal sample} with respect to the DNN $f$ if $f(\mathbf{x})= c_\mathbf{x}$. Notice that under our definition, those samples in the training dataset which are wrongly labeled by $f$ are also adversarial samples. %To distinguish the two cases, we refer to as \textit{``wrongly labeled (WL)''} later.

\subsection{Attacking through Adversarial Samples}
Since Szegedy \emph{et al.} made an intriguing discovery that neural networks are vulnerable to adversarial examples in~\cite{Szegedy2013Intriguing}, many methods have been developed on how to generate adversarial samples efficiently (e.g., with minimum perturbation). That is, given a normal sample $\mathbf{x}$, an attacker aims to find a minimum perturbation $\Delta\mathbf{x}$ which satisfies $f(\mathbf{x}+\mathbf{\Delta}\mathbf{x})\neq c_\mathbf{x}$. In this section, we briefly introduce several state-of-the-art attacking algorithms. \\

\noindent \textbf{FGSM}: The Fast Gradient Sign Method (FGSM)~\cite{FGSM} is designed based on the intuition that we can change the label of an input sample by changing its softmax value to the largest extent, which is represented by its gradient.
% explanation of the neural networks’ vulnerability that it is its linear nature that makes a neural network easy to be misled instead of the nonlinearity and overﬁtting. If the softmax score of a class linearly has to do with the input, we could just linearly modify
% the input to make the softmax score of the true label decrease.  
% With, 
The implementation of FGSM is straightforward and efficient. By simply adding up the sign of gradient of the cost function with respect to the input, we could quickly obtain a potential adversarial counterpart of a normal sample by the follow formulation:
\[
    \mathbf{\Hat{x}}=\mathbf{x}+{\epsilon}\mathbf{sign}(\nabla{\mathbf{J}(\mathbf{\theta},\mathbf{x},c_\mathbf{x})})
\]
, where $\mathbf{J}$ is the cost used to train the model, $\mathbf{\theta}$ is the parameters. %and $y$ is the true class of $\mathbf{x}$.  
Notice that FGSM can not guarantee the adversarial perturbation is minimal. \\
% though it is an efficient manner. 

\noindent \textbf{JSMA}: Jacobian-based Saliency Map Attack(JSMA)~\cite{JSMA} is devised to attack one model with minimal perturbations and enable the adversarial samples to mislead the target model into classifying it with certain (attacker-desired) label. It is a greedy algorithm that changes one pixel during each iteration to increase probability of having the target label. Based on the Jacobian matrix, they calculate a saliency map to model the impact that each pixel imposes on the target classification. With the saliency map, the algorithm picks the pixel which may have the most significant influence on the desired changes and then increases it to the max value. The process is repeated until it reaches one of the stopping criteria, i.e., the number of pixels modified has reached the bound, or the target label has been achieved. Define

\begin{equation}
\left\{
    \begin{aligned}
       a_i = & \frac{\partial{\mathbf{F_t}(\mathbf{X})}}{\partial{X_i}}\\
       b_i = & \sum_{k \neq t}\frac{\partial{\mathbf{F_k}(\mathbf{X})}}{\partial{X_i}}\nonumber 
    \end{aligned}
\right.
\end{equation}

Then, the saliency map at each iteration is defined as follow:

\begin{equation}
   S(\mathbf{X},t)_i =  \left\{
   \begin{aligned} 
    & a_i\times\left|b_i\right| & if \; a_i>0\; and\; b_i<0 \\
    & 0 & otherwise  \\
   \end{aligned}
   \right.  \nonumber
\end{equation}

However, it is too strict to select one pixel at a time because quite few pixels could meet that definition. Thus, instead of picking one pixel at a time, the authors proposed to pick two
pixels to modify according to the follow objective: 
\[
\arg\max_{(p_1,p_2)} \left( \frac{\partial{\mathbf{F}_t(\mathbf{X})}}{\partial{\mathbf{X}_{p_1}}} + \frac{\partial{\mathbf{F}_t(\mathbf{X})}}{\partial{\mathbf{X}_{p_2}}} \right)\times \left|\sum_{i=p_1,p_2}\sum_{k \neq t} \frac{\partial{\mathbf{F}_k(\mathbf{X})}}{\partial{\mathbf{X}_{i}}}    \right| 
\]
where$(p_1,p_2)$ is the candidate pair, and $t$ is the target class.

JSMA is relatively time-consuming and memory-consuming since it needs to compute the Jacobian matrix and pick out a pair from nearly $\binom{n}{2}$ candidate pairs at each iteration. \\

% Remind, there is a decreased-counterpart of the saliency map defined above, but they are  
\noindent \textbf{DeepFool}:
The idea of DeepFool (DF) is to make the normal samples cross the decision boundary with minimum perturbations~\cite{DeepFool}. The authors first deduced an iterative algorithm for binary classiﬁers with Taylor's Formula, and then analytically derived the solution for multiclass classiﬁers. The exact derivation process is complicated and thus we refer the reader to~\cite{DeepFool} for details. \\

\noindent \textbf{C\&W}:
Carlini \emph{et al.}~\cite{CW} proposed a group of attacks based on three distance metrics. The key idea is to solve an optimization problem which minimizes the perturbation imposed on the normal sample (with certain distance metric) and maximizes the probability of the target class label. 
% Note, JSMA minimizes the perturbations by restricting the number of pixels which need to be changed while C\&W does this by minimizing the total changes of all pixels. 
% They designs a series of loss functions to make the desired class's probability as large as possible. 
The objective function is as follow:
\[
    \arg\min \Delta\mathbf{x} + c\cdot f(\hat{\mathbf{x}},t)
\]
where $\Delta\textbf{x}$ is according to some distance metric, e.g, $L_0$, $L_2$, $L_{\infty}$, $\hat{x}=\mathbf{x}+\Delta\mathbf{x}$ is the clipped adversarial sample and $t$ is its target label. They devised a clip function for the adversarial sample such that the value of each pixel dose not exceed the legal range. The clip function and the best loss function the authors claimed are shown as follows.
\begin{equation}
\begin{aligned}
clip:& \hat{\mathbf{x}} &=& 0.5(tanh(\tilde{\mathbf{x}})+1) \\ \nonumber
loss:& f(\hat{\mathbf{x}},t) &=& \max(\max\{G(\hat{\mathbf{x}})_c:c \neq t\}-G(\hat{\mathbf{x}})_t, 0) 
\end{aligned}
\end{equation}
where $G(\mathbf{x})$ denotes the output vector of a model and $t$ is the target class. Readers can refer to~\cite{CW} for details. \\
% $\gamma$ is an hyperparameter which encourages the solver to ﬁnd an adversarial samples with high conﬁdence. 

\noindent \textbf{Black-Box}: All the above mentioned attacks are white-box attacks which means that the attackers require the full knowledge of the DNN model. Black-Box (BB) attack only needs to know the output of the DNN model given a certain input sample. The idea is to train a substitute model to mimic the behaviors of the targeted model with data augmentation. Then, it applies one of the existing attack algorithm, e.g., FGSM and JSMA, to generate adversarial samples for the substitute model. The key assumption to its success is that the adversarial samples transfer between different model architectures~\cite{Szegedy2013Intriguing,FGSM}. 

\subsection{Problem Definition}
Observing that adversarial samples are relatively easy to craft, a variety of defense mechanisms against adversarial samples have been proposed~\cite{,,,}, as we have briefly introduced in Section~\ref{sec:intr}. However, in~\cite{}, XXX \emph{et al.} systematically evaluated the state-of-the-art defense mechanisms and shows that most of them are ineffective against the state-of-the-art attacking methods. In this work, we take a complementary perspective and propose to detect adversarial samples at runtime. \textit{The problem is: given an input sample $\mathbf{x}$ to a deployed DNN $f$, how can we efficiently and correctly decide whether $f(\mathbf{x})=c_\mathbf{x}$ (i.e., a normal sample) or not (i.e., an adversarial sample)?} If we know that $\mathbf{x}$ is likely an adversarial sample, we could raise an alarm for further investigation. Furthermore, can we quantify our confidence on the drawn conclusion?
